Fully Sparse Fusion for 3D Object Detection

Currently prevalent multimodal 3D detection methods are built upon LiDAR-based detectors that usually use dense Bird's-Eye-View (BEV) feature maps. However, the cost of such BEV feature maps is quadratic to the detection range, making it not suitable for long-range detection. Fully sparse architecture is gaining attention as they are highly efficient in long-range perception. In this paper, we study how to effectively leverage image modality in the emerging fully sparse architecture. Particularly, utilizing instance queries, our framework integrates the well-studied 2D instance segmentation into the LiDAR side, which is parallel to the 3D instance segmentation part in the fully sparse detector. This design achieves a uniform query-based fusion framework in both the 2D and 3D sides while maintaining the fully sparse characteristic. Extensive experiments showcase state-of-the-art results on the widely used nuScenes dataset and the long-range Argoverse 2 dataset. Notably, the inference speed of the proposed method under the long-range LiDAR perception setting is 2.7 $\times$ faster than that of other state-of-the-art multimodal 3D detection methods. Code will be released at \url{https://github.com/BraveGroup/FullySparseFusion}.

==> tables/abl_ground_plane_points.tex <==
\begin{table}[H]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|ccccc}
\toprule
Ground-plane points & mAP~$\uparrow$  & NDS~$\uparrow$  & mATE~$\downarrow$  & mASE~$\downarrow$  & mAOE~$\downarrow$  & mAVE~$\downarrow$  & mAAE~$\downarrow$  \\ \midrule
\textbf{$\times$} & 70.4 & 72.7 & 0.277 & 0.247 & 0.317 & 0.218 & 0.186 \\
\checkmark        & 70.4 & 72.8 & 0.283 & 0.240 & 0.305 & 0.219 & 0.185 \\ \bottomrule
\end{tabular}
}
\end{center}
\caption{Ablation study on the influence of ground-plane points in our model.}
\label{tab:ground_plane_points}
\end{table}

==> tables/abl_lidar_backbone.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c|cc}
\toprule
Channel Scaling Factor & mAP & NDS \\
\midrule
1/2 & 68.8 & 70.4 \\
1 & 70.4 & 72.7 \\
2 & 70.9 & 73.8 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Ablation Study on the influence of LiDAR backbone in our model.}
\label{tab:backbone_channel}
\end{table}

